P4Kube: In-Network Load Balancer for Kubernetes

Kubernetes Services such as LoadBalancer and NodePort expose applications running on pods within a Kubernetes cluster to external users. While the LoadBalancer Service requires an external load-balancing middleware, its alternative, NodePort Service, adds additional hops on the path between clients and the worker nodes. In this paper, we propose P4Kube, a framework consisting of a P4 data plane program and a Kubernetes plugin. Our solution effectively performs load balancing of requests to the worker nodes of a cluster based on the number of running replicas. In P4Kube, the data packets completely bypass the system's control plane. Unlike the previous work, to update its state, the P4Kube data plane works directly with the Kubernetes control plane without any involvement of the network control plane. Our experiments show up to 50% improvement in the average request time to the cluster compared to conventional approaches.

==> bg.tex <==
\section{Background}
\label{sec:bg}

% The need for green data center computing in detail
% The main sources of data consumption in data centers
% The weight of server and network components
% What is the fundamental approach and has it has been done
% Why programmability might be a key solution
\textbf{Data Center Topology:}
%Data centers are the core components of the globally shared computing infrastructure. The demand for data centers service continues to grow~\cite{koot2021usage}. Data centers' traffic load varies throughout the day, month, and year. 
The data center equipment is provisioned for peak workloads, thus many of its computational and communication resources are idle most of the time~\cite{popoola2018energy}. The data storage and processing servers are often replicated and placed in different geographical locations. The communication resources, i.e., switches and links, are connected following one of the common data center topologies, such as a three-tier or fat tree. Both topologies put switches into three categories:
\begin{enumerate}
    \item \textit{Core switches}, high capacity switches connecting the data center network with the Internet;
    \item \textit{Access switches}, lower capacity switches with a high port density that are directly connected to the servers;
    \item \textit{Aggregation switches}, that forward traffic between core and access switches.
\end{enumerate}
\begin{comment}
\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{fig/fattree.eps}
		\caption{\label{fig:fatree}A typical data center topology}
	\end{center}
 \vspace{-5mm}
\end{figure}  
\end{comment}
Figure~\ref{fig:mininet} shows a simplified fat-tree topology of a data center. It can be seen that the connection between the core switch and the access switches will exist even if there is only one enabled aggregation switch between them. The increased number of aggregation switches enables the distribution of heavy flows across multiple paths during peak loads. 

\textbf{Green Computing in Data Centers: }
According to the US Department of Energy, data center facilities are one of the most energy-hungry and account for 2\% of the total US energy use~\cite{usdeptenergy}. The recent analysis of trends in demand and technological innovations predicts exponential growth in data centers' energy consumption~\cite{koot2021usage}. This growth will inevitably increase greenhouse gas emissions. Recent studies show that the current emissions are equal to or even surpass the amounts of emissions by the airline industry~\cite{engie}.

The contributors to energy consumption at data centers belong to three categories: the IT infrastructure (servers, storage, and network components), cooling, and power distribution systems. In~\cite{rong2016optimizing}, authors present the breakdown of energy consumption by a data center, in which 40\% are attributed to servers, 5\% to network equipment, 5\% to storage, 10\% to power supply systems, and 40\% to refrigeration systems. While the energy efficiency of non-IT components of data centers improves, the share of IT infrastructure in energy consumption is expected to increase. In the meantime, higher energy consumption by IT infrastructure leads to an increase in consumption in other categories. For example, network switches have high heat dissipation~\cite{popoola2018energy}, and having more active switches requires higher intensity cooling. %Figure~\ref{fig:trends} illustrates the predicted best-case energy consumption trends for non-IT and IT infrastructure in the nearest future.

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=1\columnwidth]{fig/energy_trends}
% 		\caption{\label{fig:trends}Energy consumption trends for IT and non-IT data center infrastructure in the best-case scenario~\cite{koot2021usage}}
% 	\end{center}
% \end{figure}

%The mitigation of energy consumption of data centers has benefits such as carbon footprint reduction and decreasing data center operational expenses. 
Apart from upgrading IT hardware, the major approach to decrease the IT infrastructure energy consumption is to consolidate computation and traffic and eliminate servers and switches processing light traffic~\cite{mahadevan2011energy}. These resources are usually provisioned for peak workloads and are idle most of the time while consuming considerable amounts of energy. In the meantime, the traffic consolidation should not degrade the quality of service by increasing congestion at the active network paths; neither it should increase latency by increasing the number of hops in those paths. 

Using renewable energy is a complementary measure to the overall reduction of energy consumption, and requires dynamic migration of workloads to servers that have available green energy resources~\cite{grigoryan2018grasp, siddik2021environmental, zheng2020mitigating}.  Both traffic consolidation and migration are facilitated when using Software-Defined Networking (SDN) technologies, that allow programming the control and data plane of the network switches that forward traffic in data centers.

%\subsection{Software-Defined Networking and Programmable Data Plane}
%Software-Defined Networking (SDN) is the technology that enables decoupling the control plane of a switch from its data plane. The control plane is responsible for configuring a switch (e.g., managing a forwarding table), while the data plane is responsible for forwarding the packets from an ingress port to an egress port and rewriting packet headers. In a traditional SDN, the control plane is fully programmable and can modify the switch configuration via data plane API (such as OpenFlow~\cite{mckeown2008openflow}), while the data plane simply forwards the packet according to that configuration following the standard network protocol rules. The emerging technologies of the programmable data plane, such as P4 language~\cite{bosshart2014p4}, go further by allowing a limited programmability of certain components of the data plane, such as the packet parser and ingress/egress pipelines.

%Below we discuss OpenFlow and P4 and existing green data center solutions that leverage these technologies.

\textbf{OpenFlow for Green Data Centers:} OpenFlow protocol was introduced in~\cite{mckeown2008openflow} for a programmable SDN controller of a switch to manage the forwarding tables in the data plane. OpenFlow bridged the gap between applications and networks since forwarding decisions were no longer depending solely on standard routing protocols. In ElasticTree~\cite{heller2010elastictree}, authors leveraged OpenFlow to consolidate data center traffic in the least number of switches as possible. OpenFlow was used to pull statistics from the data planes of switches to the centralized control plane, calculate the optimal paths for packets at the control plane and push the corresponding rules back into the data plane. One disadvantage of such an approach is dependence of the forwarding (i.e., data) plane on the centralized control plane; in case of a failure of the control plane the energy-efficient load balancing will be disrupted. 

% tell what's wrong with elastictree

% Talk about Elastictree, GRASP?

\textbf{Leveraging P4:} OpenFlow has several shortcomings: it is compatible only with a limited number of packet header definitions and does not allow user-defined in-data plane computations. Offloading packet processing to the SDN control plane has scalability and security issues~\cite{karakus2017survey}. P4, a language for programming packet processors, allows defining arbitrary packet parsers and programming the ingress and egress pipelines of a switch. Compared to SDN with OpenFlow, P4 makes the data plane less dependent on the control plane which improves the efficiency, security, scalability, and robustness of networks.

As of today, there is little research into how the programmability of switches with P4 can be used to reduce the energy consumption of data center networks and increase the utilization of renewable energy. In P4Green, we present the design of a data center network that relies on P4-enabled switches to dynamically control the number of active switches to forward traffic. In the meantime, the servers in our design can control the amount of traffic they receive depending on the availability of renewable energy at those servers. P4Green has a minimal dependency on the centralized networking control plane, requiring it only at the initialization stage.


